Towards Proactively Forecasting Sentence-Specific Information Popularity within Online News Documents

Multiple studies have focused on predicting the prospective popularity of an online document as a whole, without paying attention to the contributions of its individual parts. We introduce the task of proactively forecasting popularities of sentences within online news documents solely utilizing their natural language content. We model sentence-specific popularity forecasting as a sequence regression task. For training our models, we curate InfoPop, the first dataset containing popularity labels for over 1.7 million sentences from over 50,000 online news documents. To the best of our knowledge, this is the first dataset automatically created using streams of incoming search engine queries to generate sentence-level popularity annotations. We propose a novel transfer learning approach involving sentence salience prediction as an auxiliary task. Our proposed technique coupled with a BERT-based neural model exceeds nDCG values of 0.8 for proactive sentence-specific popularity forecasting. Notably, our study presents a non-trivial takeaway: though popularity and salience are different concepts, transfer learning from salience prediction enhances popularity forecasting. We release InfoPop and make our code publicly available: https://github.com/sayarghoshroy/InfoPopularity

==> refs.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}
\scriptsize
\bibitem{pop_time_ser}
Ahmed, M., Spagna, S., Huici, F., Niccolini, S.: A peek into the future:
  Predicting the evolution of popularity in user generated content. In: WSDM.
  pp. 607--616 (2013)

\bibitem{snippet_3}
Chen, W.F., Syed, S., Stein, B., Hagen, M., Potthast, M.: Abstractive snippet
  generation. WWW  (2020)

\bibitem{gru}
Chung, J., Gulcehre, C., Cho, K., Bengio, Y.: Empirical evaluation of gated
  recurrent neural networks on sequence modeling (2014)

\bibitem{bert}
Devlin, J., Chang, M.W., Lee, K., Toutanova, K.: Bert: Pre-training of deep
  bidirectional transformers for language understanding. arXiv:1810.04805
  (2018)

\bibitem{cross_task_query_based}
Egonmwan, E., Castelli, V., Sultan, M.A.: Cross-task knowledge transfer for
  query-based text summarization. In: Workshop on MRQA. pp. 72--77 (2019)

\bibitem{LexRank}
Erkan, G., Radev, D.R.: Lexrank: Graph-based lexical centrality as salience in
  text summarization. J. AI Research  \textbf{22},  457--479 (2004)

\bibitem{domain_adapt}
Gururangan, S., Marasovi{\'c}, A., Swayamdipta, S., Lo, K., Beltagy, I.,
  Downey, D., Smith, N.A.: Don't stop pretraining: adapt language models to
  domains and tasks. arXiv:2004.10964  (2020)

\bibitem{snippet_q_2}
He, J., Duboue, P., Nie, J.Y.: Bridging the gap between intrinsic and perceived
  relevance in snippet generation. In: COLING. pp. 1129--1146 (2012)

\bibitem{seq_label_survey}
He, Z., Wang, Z., Wei, W., Feng, S., Mao, X., Jiang, S.: A survey on recent
  advances in sequence labeling from deep learning models (2020)

\bibitem{cnn_dm_hermann}
Hermann, K.M., Kociský, T., Grefenstette, E., Espeholt, L., Kay, W., Suleyman,
  M., Blunsom, P.: Teaching machines to read and comprehend. In: NIPS. pp.
  1693--1701 (2015)

\bibitem{distilsum}
Jia, R., Cao, Y., Shi, H., Fang, F., Liu, Y., Tan, J.: Distilsum: Distilling
  the knowledge for extractive summarization. In: CIKM. pp. 2069--–2072
  (2020)

\bibitem{predicting_pop}
Keneshloo, Y., Wang, S., Han, E., Ramakrishnan, N.: Predicting the popularity
  of news articles. In: SDM (2016)

\bibitem{predict_news_headline_pop}
Lamprinidis, S., Hardt, D., Hovy, D.: Predicting news headline popularity with
  syntactic and semantic knowledge using multi-task learning. In: EMNLP. pp.
  659--664 (2018)

\bibitem{time_pop}
Liao, D., Xu, J., Li, G., Huang, W., Liu, W., Li, J.: Popularity prediction on
  online articles with deep fusion of temporal process and content features.
  In: AAAI (2019)

\bibitem{bertsumm}
Liu, Y.: Fine-tune bert for extractive summarization. arXiv:1903.10318  (2019)

\bibitem{presumm}
Liu, Y., Lapata, M.: Text summarization with pretrained encoders. In:
  EMNLP-IJCNLP. pp. 3730--3740 (2019)

\bibitem{roberta}
Liu, Y., Ott, M., Goyal, N., Du, J., Joshi, M., Chen, D., Levy, O., Lewis, M.,
  Zettlemoyer, L., Stoyanov, V.: Roberta: A robustly optimized bert pretraining
  approach (2019)

\bibitem{textrank}
Mihalcea, R., Tarau, P.: Textrank: Bringing order into text. In: EMNLP. pp.
  404--411 (2004)

\bibitem{multi_source_social}
Moniz, N., Torgo, L.: Multi-source social feedback of online news feeds.
  arXiv:1801.07055  (2018)

\bibitem{summarunner}
Nallapati, R., Zhai, F., Zhou, B.: Summarunner: A recurrent neural network
  based sequence model for extractive summarization of documents.
  arXiv:1611.04230  (2016)

\bibitem{stilts}
Phang, J., F{\'e}vry, T., Bowman, S.R.: Sentence encoders on stilts:
  Supplementary training on intermediate labeled-data tasks. arXiv preprint
  arXiv:1811.01088  (2018)

\bibitem{petition_time}
Proskurnia, J., Grabowicz, P.A., Kobayashi, R., Castillo, C.,
  Cudr{\'e}-Mauroux, P., Aberer, K.: Predicting the success of online petitions
  leveraging multidimensional time-series. WWW  (2017)

\bibitem{intermediate_TL}
Pruksachatkun, Y., Phang, J., Liu, H., Htut, P.M., Zhang, X., Pang, R.Y.,
  Vania, C., Kann, K., Bowman, S.R.: Intermediate-task transfer learning with
  pretrained language models: When and why does it work? In: ACL (2020)

\bibitem{news_article_pop}
Pugachev, A., Voronov, A., Makarov, I.: Prediction of news popularity via
  keywords extraction and trends tracking. Recent Trends in Analysis of Images,
  Social Networks and Texts  \textbf{1357},  37--51 (2020)

\bibitem{predict_mining}
Rizos, G., Papadopoulos, S., Kompatsiaris, Y.: Predicting news popularity by
  mining online discussions. In: WWW. pp. 737--742 (2016)

\bibitem{neural_abs_summ}
Rush, A.M., Chopra, S., Weston, J.: A neural attention model for abstractive
  sentence summarization (2015)

\bibitem{pop_headline_gen}
Song, Y.Z., Shuai, H.H., Yeh, S.L., Wu, Y.L., Ku, L.W., Peng, W.C.: Attractive
  or faithful? popularity-reinforced learning for inspired headline generation.
  In: AAAI. vol.~34, pp. 8910--8917 (2020)

\bibitem{petition_pop}
Subramanian, S., Baldwin, T., Cohn, T.: Content-based popularity prediction of
  online petitions using a deep regression model. In: ACL. pp. 182--188 (2018)

\bibitem{ranking_news_pop}
Tatar, A., Antoniadis, P., De~Amorim, M.D., Fdida, S.: Ranking news articles
  based on popularity prediction. In: ASONAM. pp. 106--110 (2012)

\bibitem{pop_content_meta}
Uddin, M.T., Patwary, M.J.A., Ahsan, T., Alam, M.S.: Predicting the popularity
  of online news from content metadata. In: ICISET. pp.~1--5 (2016)

\bibitem{transformer}
Vaswani, A., Shazeer, N., Parmar, N., Uszkoreit, J., Jones, L., Gomez, A.N.,
  Kaiser, {\L}., Polosukhin, I.: Attention is all you need. In: NIPS. pp.
  5998--6008 (2017)

\bibitem{glue}
Wang, A., Singh, A., Michael, J., Hill, F., Levy, O., Bowman, S.R.: {GLUE}: A
  multi-task benchmark and analysis platform for natural language
  understanding. arXiv preprint arXiv:1804.07461  (2018)

\bibitem{catboost}
Wang, K., Wang, P., Chen, X., Huang, Q., Mao, Z., Zhang, Y.: A feature
  generalization framework for social media popularity prediction. In: ACM MM.
  pp. 4570--4574 (2020)

\bibitem{seq_pred_soc_comp}
Wu, B., Cheng, W.H., Zhang, Y., Huang, Q., Li, J., Mei, T.: Sequential
  prediction of social media popularity with deep temporal context networks.
  arXiv:1712.04443  (2017)

\bibitem{time_matters}
Wu, B., Cheng, W.H., Zhang, Y., Mei, T.: Time matters: Multi-scale
  temporalization of social media popularity. In: ACM MM. pp. 1336--1344 (2016)

\bibitem{temp_dyn_flickr}
Wu, B., Mei, T., Cheng, W.H., Zhang, Y.: Unfolding temporal dynamics:
  Predicting social media popularity using multi-scale temporal decomposition.
  In: AAAI. p. 272–278 (2016)

\bibitem{hibert}
Zhang, X., Wei, F., Zhou, M.: Hibert: Document level pre-training of
  hierarchical bidirectional transformers for document summarization (2019)

\bibitem{text_match}
Zhong, M., Liu, P., Chen, Y., Wang, D., Qiu, X., Huang, X.: Extractive
  summarization as text matching. In: ACL. pp. 6197--6208 (2020)
  
\bibitem{forecast_pop_news}
Voronov, A and Shen, Y and Mondal, PK:
Forecasting Popularity of News Article by Title Analyzing with BN-LSTM Network. In: ICDMML. pp. 19--27 (2019)

\bibitem{movie_pop}
Abidi, R and Xu, Y and Ni, J and Xiangmeng, W and Zhang, W: Popularity prediction of movies: from statistical modeling to machine learning techniques. In Multimedia Tools and Applications. pp. 1-35 (2020)

\bibitem{time-aware-movie}
Ji, Y and Sun, A and Zhang, J and Li, C: A Re-Visit of the Popularity Baseline in Recommender Systems. In SIGIR. pp. 1749--1752 (2020)

\bibitem{entity_pop}
Chen, A and Gudipati, P and Longpre, S  and Ling, X  and Singh, S: Evaluating Entity Disambiguation and the Role of Popularity in Retrieval-Based NLP. In ACL-IJCNLP. pp. 4472--4485 (2021)

\bibitem{bart}
Lewis, Mike  and
      Liu, Y  and
      Goyal, N  and
      Ghazvininejad, M  and
      Mohamed, A  and
      Levy, O  and
      Stoyanov, V  and
      Zettlemoyer, L: BART: Denoising Sequence-to-Sequence Pre-training for Natural Language Generation, Translation, and Comprehension. In ACL. pp. 7871--7880 (2020)
      
\bibitem{cross_task_spanrep}
Toshniwal, S  and
      Shi, H and
      Shi, B  and
      Gao, L  and
      Livescu, K  and
      Gimpel, K: A Cross-Task Analysis of Text Span Representations. In: Workshop on Representation Learning for NLP, ACL. pp. 166--176 (2020)
    
\bibitem{docret}
Hofstätter, S and Mitra, B and Zamani, H and Craswell, N and Hanbury, A: Intra-Document Cascading: Learning to Select Passages for Neural Document Ranking. In SIGIR. pp. 1349--1358 (2021)

\end{thebibliography}

